The VLA/ALMA Nascent Disk and Multiplicity (VANDAM) Survey of Orion Protostars V. A Characterization of Protostellar Multiplicity

We characterize protostellar multiplicity in the Orion molecular clouds using ALMA 0.87~mm and VLA 9~mm continuum surveys toward 328 protostars. These observations are sensitive to projected spatial separations as small as $\sim$20~au, and we consider source separations up to 10$^4$~au as potential companions. The overall multiplicity fraction (MF) and companion fraction (CF) for the Orion protostars are 0.30$\pm$0.03 and 0.44$\pm$0.03, respectively, considering separations from 20 to 10$^4$~au. The MFs and CFs are corrected for potential contamination by unassociated young stars using a probabilistic scheme based on the surface density of young stars around each protostar. The companion separation distribution as a whole is double peaked and inconsistent with the separation distribution of solar-type field stars, while the separation distribution of Flat Spectrum protostars is consistent solar-type field stars. The multiplicity statistics and companion separation distributions of the Perseus star-forming region are consistent with those of Orion. Based on the observed peaks in the Class 0 separations at $\sim$100~au and $\sim$10$^3$~au, we argue that multiples with separations $<$500~au are likely produced by both disk fragmentation and turbulent fragmentation with migration, and those at $\ga$10$^3$~au result primarily from turbulent fragmentation. We also find that MFs/CFs may rise from Class 0 to Flat Spectrum protostars between 100 and 10$^3$~au in regions of high YSO density. This finding may be evidence for migration of companions from $>$10$^3$~au to $<$10$^3$~au, and that some companions between 10$^3$ and 10$^4$~au must be (or become) unbound.

==> multiples-input-catalog-orion.tex <==
HH270VLA1-A & HH270VLA1 & 05:51:34.587 & +02:56:46.01 & 7.34 & 32.00 & 0 & 2.2 & 430.1\\
HH270VLA1-B & HH270VLA1 & 05:51:34.600 & +02:56:45.88 & 7.34 & 32.00 & 0 & 2.2 & 430.1\\
HH270mms1-B & HH270mms1 & 05:51:22.632 & +02:56:06.80 & 7.74 & 72.00 & I & 2.2 & 405.7\\
HH270mms1-A & HH270mms1 & 05:51:22.717 & +02:56:04.98 & 7.74 & 72.00 & I & 2.2 & 405.7\\
HH270mms2 & HH270mms2 & 05:51:22.572 & +02:55:43.16 & 4.55 & 249.00 & Flat & 2.2 & 413.3\\
HH111MMS-B & HH111MMS & 05:51:46.066 & +02:48:30.80 & 21.98 & 78.00 & I & 2.2 & 410.6\\
HH111MMS-A & HH111MMS & 05:51:46.253 & +02:48:29.65 & 21.98 & 78.00 & I & 2.2 & 410.6\\
HOPS-367 & HOPS-367 & 05:54:36.287 & +01:53:54.06 & 0.03 & 249.40 & I & 2.1 & 354.9\\
HOPS-7 & HOPS-7 & 05:54:20.057 & +01:50:42.64 & 0.38 & 58.00 & 0 & 3.5 & 357.1\\
HOPS-5 & HOPS-5 & 05:54:32.163 & +01:48:07.08 & 0.28 & 187.10 & I & 6.0 & 354.6\\
HOPS-4 & HOPS-4 & 05:54:53.789 & +01:47:09.70 & 0.30 & 203.30 & I & 2.6 & 351.6\\
HOPS-354 & HOPS-354 & 05:54:24.262 & +01:44:19.91 & 4.70 & 34.80 & 0 & 7.9 & 355.4\\
HOPS-3 & HOPS-3 & 05:54:56.963 & +01:42:56.23 & 0.39 & 467.50 & Flat & 1.7 & 351.0\\
HOPS-2 & HOPS-2 & 05:54:09.137 & +01:42:51.70 & 0.39 & 356.50 & I & 23.3 & 357.4\\
HOPS-1 & HOPS-1 & 05:54:12.347 & +01:42:35.48 & 1.10 & 72.60 & I & 17.9 & 356.9\\
2MJ05474500+0038418-A & 2MJ05474500+0038418-A & 05:47:44.999 & +00:38:41.89 & -99.00 & -99.00 & Unclassified & 13.9 & 400.0\\
2MJ05474500+0038418-B & 2MJ05474500+0038418-B & 05:47:44.960 & +00:38:41.82 & -99.00 & -99.00 & Unclassified & 13.9 & 400.0\\
HOPS-345 & HOPS-345 & 05:47:38.966 & +00:38:36.21 & 0.49 & 219.40 & I & 25.5 & 430.7\\
HOPS-406 & HOPS-406 & 05:47:43.434 & +00:38:21.31 & 0.50 & 24.60 & 0 & 16.4 & 430.3\\
HOPS-344 & HOPS-344 & 05:47:24.735 & +00:37:34.83 & 0.10 & 408.20 & I & 9.7 & 431.4\\
HOPS-343 & HOPS-343 & 05:47:59.041 & +00:35:32.83 & 4.07 & 82.10 & I & 4.8 & 427.6\\
HOPS-342 & HOPS-342 & 05:47:57.108 & +00:35:27.12 & 0.34 & 312.60 & I & 5.3 & 427.8\\
HOPS-404 & HOPS-404 & 05:48:07.714 & +00:33:51.83 & 1.00 & 26.10 & 0 & 2.4 & 430.1\\
HOPS-340 & HOPS-340 & 05:47:01.311 & +00:26:23.04 & 1.95 & 40.60 & 0 & 25.7 & 430.9\\
HOPS-341 & HOPS-341 & 05:47:00.914 & +00:26:21.49 & 2.18 & 39.40 & 0 & 25.4 & 430.9\\
HOPS-338-B & HOPS-338 & 05:46:57.302 & +00:23:57.97 & 0.22 & 53.70 & 0 & 50.0 & 430.7\\
HOPS-338-A & HOPS-338 & 05:46:57.356 & +00:23:50.43 & 0.22 & 53.70 & 0 & 50.0 & 430.7\\
HOPS-337 & HOPS-337 & 05:46:55.092 & +00:23:34.55 & 0.94 & 128.80 & I & 45.7 & 430.7\\
HOPS-336 & HOPS-336 & 05:46:02.278 & +00:23:30.60 & 0.03 & 164.60 & I & 6.2 & 430.5\\
HOPS-393 & HOPS-393 & 05:46:42.485 & +00:23:01.13 & 0.07 & 250.50 & I & 17.6 & 430.7\\
HOPS-366-B & HOPS-366 & 05:47:04.009 & +00:22:10.45 & 6.77 & 292.20 & I & 145.7 & 430.5\\
HOPS-366-A & HOPS-366 & 05:47:04.003 & +00:22:10.33 & 6.77 & 292.20 & I & 145.7 & 430.5\\
HOPS-361-H & HOPS-361 & 05:47:05.125 & +00:22:01.46 & 503.00 & 69.00 & 0 & 145.7 & 430.4\\
HOPS-361-G-A & HOPS-361 & 05:47:05.367 & +00:21:50.53 & 503.00 & 69.00 & 0 & 91.3 & 430.4\\
HOPS-361-G-B & HOPS-361 & 05:47:05.451 & +00:21:50.08 & 503.00 & 69.00 & 0 & 91.3 & 430.4\\
HOPS-361-C-B & HOPS-361 & 05:47:04.625 & +00:21:47.88 & 503.00 & 69.00 & 0 & 91.3 & 430.4\\
HOPS-361-C-A & HOPS-361 & 05:47:04.631 & +00:21:47.85 & 503.00 & 69.00 & 0 & 91.3 & 430.4\\
HOPS-361-B & HOPS-361 & 05:47:04.755 & +00:21:45.45 & 503.00 & 69.00 & 0 & 91.3 & 430.4\\
HOPS-361-A & HOPS-361 & 05:47:04.783 & +00:21:42.86 & 503.00 & 69.00 & 0 & 91.3 & 430.4\\
HOPS-361-E-B & HOPS-361 & 05:47:04.622 & +00:21:41.34 & 434.46 & 69.00 & 0 & 91.3 & 400.0\\
HOPS-361-E-A & HOPS-361 & 05:47:04.624 & +00:21:41.30 & 434.46 & 69.00 & 0 & 91.3 & 400.0\\
HOPS-361-F & HOPS-361 & 05:47:04.967 & +00:21:40.74 & 503.00 & 69.00 & 0 & 91.3 & 430.4\\
HOPS-361-D & HOPS-361 & 05:47:04.317 & +00:21:38.04 & 503.00 & 69.00 & 0 & 91.3 & 430.4\\
HOPS-392 & HOPS-392 & 05:46:16.505 & +00:21:35.75 & 0.07 & 62.40 & 0 & 11.0 & 430.4\\
HOPS-361-J & HOPS-361 & 05:47:04.525 & +00:21:23.89 & 503.00 & 69.00 & 0 & 91.3 & 430.4\\
HOPS-347 & HOPS-347 & 05:47:15.947 & +00:21:22.89 & 0.56 & 33.50 & 0 & 57.1 & 430.2\\
HOPS-361-I & HOPS-361 & 05:47:04.246 & +00:21:22.70 & 503.00 & 69.00 & 0 & 91.3 & 430.4\\
HOPS-365 & HOPS-365 & 05:47:10.613 & +00:21:13.71 & 20.26 & 160.30 & I & 121.3 & 430.3\\
HOPS-359 & HOPS-359 & 05:47:24.840 & +00:20:59.39 & 10.45 & 36.70 & 0 & 56.5 & 429.4\\
HOPS-390 & HOPS-390 & 05:47:32.455 & +00:20:21.64 & 3.38 & 54.30 & 0 & 44.7 & 428.4\\
HOPS-364-B & HOPS-364 & 05:47:36.554 & +00:20:06.00 & 34.26 & 96.70 & I & 22.6 & 427.8\\
HOPS-364-A & HOPS-364 & 05:47:36.563 & +00:20:05.92 & 34.26 & 96.70 & I & 22.6 & 427.8\\
HOPS-331 & HOPS-331 & 05:46:28.337 & +00:19:49.33 & 0.36 & 82.50 & Flat & 11.9 & 430.3\\
HOPS-407 & HOPS-407 & 05:46:28.251 & +00:19:27.96 & 0.71 & 26.80 & 0 & 11.5 & 419.1\\
HOPS-329 & HOPS-329 & 05:47:01.601 & +00:17:58.92 & 2.56 & 89.20 & I & 41.9 & 430.2\\
HOPS-326 & HOPS-326 & 05:46:39.554 & +00:04:16.87 & 0.57 & 58.80 & 0 & 47.5 & 428.8\\
HOPS-325 & HOPS-325 & 05:46:39.199 & +00:01:12.31 & 6.46 & 49.20 & 0 & 50.5 & 428.5\\
HOPS-363-A & HOPS-363 & 05:46:43.122 & +00:00:52.35 & 23.36 & 367.60 & Flat & 50.1 & 428.4\\
HOPS-363-B & HOPS-363 & 05:46:43.132 & +00:00:52.25 & 23.36 & 367.60 & Flat & 50.1 & 428.4\\
HOPS-324 & HOPS-324 & 05:46:37.566 & +00:00:33.83 & 2.33 & 89.90 & I & 32.9 & 428.4\\
HOPS-389-B & HOPS-389 & 05:46:46.604 & +00:00:29.52 & 6.20 & 42.80 & 0 & 37.9 & 428.4\\
HOPS-389-A & HOPS-389 & 05:46:47.019 & +00:00:27.07 & 6.20 & 42.80 & 0 & 37.9 & 428.4\\
HOPS-323-A & HOPS-323 & 05:46:47.697 & +00:00:25.27 & 10.27 & 82.90 & I & 33.0 & 428.4\\
HOPS-323-B & HOPS-323 & 05:46:47.667 & +00:00:24.81 & 10.27 & 82.90 & I & 33.0 & 428.4\\
HOPS-322 & HOPS-322 & 05:46:46.517 & +00:00:16.09 & 0.50 & 71.30 & I & 41.9 & 428.3\\
HOPS-321 & HOPS-321 & 05:46:33.172 & +00:00:02.03 & 3.89 & 78.60 & I & 23.3 & 428.4\\
HOPS-403 & HOPS-403 & 05:46:27.906 & -00:00:52.15 & 4.30 & 43.90 & 0 & 34.1 & 428.2\\
HOPS-373-A & HOPS-373 & 05:46:31.099 & -00:02:33.02 & 5.53 & 36.90 & 0 & 34.1 & 428.1\\
HOPS-373-B & HOPS-373 & 05:46:30.905 & -00:02:35.19 & 5.53 & 36.90 & 0 & 34.1 & 428.1\\
HOPS-320 & HOPS-320 & 05:46:14.212 & -00:05:26.81 & 0.46 & 87.00 & I & 26.7 & 427.7\\
HOPS-388 & HOPS-388 & 05:46:13.140 & -00:06:04.90 & 27.65 & 321.90 & Flat & 29.0 & 427.7\\
HOPS-318 & HOPS-318 & 05:46:13.521 & -00:08:55.93 & 0.15 & 312.60 & Flat & 47.5 & 427.3\\
HOPS-386-C & HOPS-386 & 05:46:08.923 & -00:09:56.12 & 23.40 & 147.40 & I & 41.1 & 427.2\\
HOPS-387-A & HOPS-387 & 05:46:07.838 & -00:09:59.59 & 5.58 & 118.30 & I & 39.0 & 427.2\\
HOPS-386-B & HOPS-386 & 05:46:08.429 & -00:10:00.52 & 23.40 & 147.40 & I & 41.1 & 427.2\\
HOPS-387-B & HOPS-387 & 05:46:07.856 & -00:10:01.30 & 5.58 & 118.30 & I & 39.0 & 427.2\\
HOPS-386-A & HOPS-386 & 05:46:08.487 & -00:10:03.05 & 23.40 & 147.40 & I & 41.1 & 427.2\\
HOPS-317-A & HOPS-317 & 05:46:08.597 & -00:10:38.49 & 4.92 & 47.50 & 0 & 29.6 & 427.1\\
HOPS-317-B & HOPS-317 & 05:46:08.376 & -00:10:43.65 & 4.92 & 47.50 & 0 & 29.6 & 427.1\\
HOPS-402 & HOPS-402 & 05:46:10.031 & -00:12:16.88 & 0.57 & 24.20 & 0 & 28.8 & 426.9\\
HOPS-401 & HOPS-401 & 05:46:07.724 & -00:12:21.25 & 0.63 & 26.00 & 0 & 29.8 & 426.9\\
HOPS-358-A & HOPS-358 & 05:46:07.257 & -00:13:30.22 & 25.77 & 41.70 & 0 & 17.1 & 426.8\\
HOPS-358-B & HOPS-358 & 05:46:07.331 & -00:13:43.50 & 25.77 & 41.70 & 0 & 17.1 & 426.8\\
HOPS-385 & HOPS-385 & 05:46:04.775 & -00:14:16.68 & 12.15 & 377.10 & Flat & 11.3 & 426.7\\
HOPS-315 & HOPS-315 & 05:46:03.635 & -00:14:49.56 & 6.42 & 180.30 & I & 8.7 & 426.6\\
HH212mms & HH212mms & 05:43:51.408 & -01:02:53.16 & 13.55 & 53.00 & 0 & 2.0 & 413.2\\
HOPS-312-A & HOPS-312 & 05:43:05.690 & -01:15:54.59 & 0.73 & 46.70 & 0 & 2.0 & 416.3\\
HOPS-312-B & HOPS-312 & 05:43:05.705 & -01:15:54.83 & 0.73 & 46.70 & 0 & 2.0 & 416.3\\
HOPS-400-A & HOPS-400 & 05:42:45.246 & -01:16:13.62 & 2.88 & 35.00 & 0 & 1.7 & 415.4\\
HOPS-400-B & HOPS-400 & 05:42:45.257 & -01:16:14.03 & 2.88 & 35.00 & 0 & 1.7 & 415.4\\
HOPS-311 & HOPS-311 & 05:43:03.056 & -01:16:29.32 & 2.78 & 383.00 & Flat & 2.4 & 416.1\\
HOPS-310 & HOPS-310 & 05:42:27.677 & -01:20:01.33 & 13.46 & 51.80 & 0 & 1.3 & 414.3\\
J054227.77-012902.2 & J054227.77-012902.2 & 05:42:27.764 & -01:20:02.20 & -99.00 & -99.00 & Unclassified & 1.3 & 414.3\\
HOPS-305 & HOPS-305 & 05:41:45.386 & -01:51:56.82 & 0.94 & 300.70 & Flat & 115.8 & 409.6\\
HOPS-357-B & HOPS-357 & 05:41:39.143 & -01:52:07.29 & 14.26 & 628.20 & Flat & 211.0 & 409.4\\
HOPS-357-A & HOPS-357 & 05:41:39.128 & -01:52:07.45 & 14.26 & 628.20 & Flat & 211.0 & 409.4\\
HOPS-384-region-H & HOPS-384 & 05:41:45.902 & -01:54:11.17 & 1404.97 & 51.90 & 0 & 1185.4 & 409.5\\
2M05414611-0154147 & 2M05414611-0154147 & 05:41:46.123 & -01:54:14.99 & -99.00 & -99.00 & Unclassified & 1185.4 & 400.0\\
2M05414482-0154251 & 2M05414482-0154251 & 05:41:44.828 & -01:54:25.31 & -99.00 & -99.00 & Unclassified & 470.9 & 400.0\\
NGC2024-FIR3-B & HOPS-384 & 05:41:43.167 & -01:54:25.42 & 209.14 & -99.00 & 0 & 1185.4 & 409.5\\
NGC2024-FIR3-A & HOPS-384 & 05:41:43.087 & -01:54:26.27 & 209.14 & -99.00 & 0 & 1039.4 & 409.5\\
HOPS-384-region-D & HOPS-384 & 05:41:45.524 & -01:54:27.14 & 1404.97 & 51.90 & 0 & 1185.4 & 409.5\\
2M05414550-0154286 & 2M05414550-0154286 & 05:41:45.490 & -01:54:28.92 & -99.00 & -99.00 & Unclassified & 1185.4 & 400.0\\
2M05414580-0154297-A & 2M05414580-0154297-A & 05:41:45.810 & -01:54:30.05 & -99.00 & -99.00 & Unclassified & 1185.4 & 400.0\\
2M05414580-0154297-B & 2M05414580-0154297-B & 05:41:45.805 & -01:54:30.30 & -99.00 & -99.00 & Unclassified & 1185.4 & 400.0\\
HOPS-384-region-G & HOPS-384 & 05:41:43.915 & -01:54:34.09 & 1404.97 & 51.90 & 0 & 1039.4 & 409.5\\
2M05414325-0154343 & 2M05414325-0154343 & 05:41:43.248 & -01:54:34.35 & -99.00 & -99.00 & Unclassified & 1039.4 & 400.0\\
2M05414483-0154357 & 2M05414483-0154357 & 05:41:44.842 & -01:54:35.98 & -99.00 & -99.00 & Unclassified & 1185.4 & 400.0\\
HOPS-384-B & HOPS-384 & 05:41:44.016 & -01:54:43.14 & 1404.97 & 51.90 & 0 & 527.0 & 409.5\\
2M05414138-0154445 & 2M05414138-0154445 & 05:41:41.390 & -01:54:44.75 & -99.00 & -99.00 & Unclassified & 1039.4 & 400.0\\
HOPS-384-A-B & HOPS-384 & 05:41:44.140 & -01:54:45.97 & 1404.97 & 51.90 & 0 & 527.0 & 409.5\\
HOPS-384-A & HOPS-384 & 05:41:44.135 & -01:54:46.06 & 1404.97 & 51.90 & 0 & 527.0 & 409.5\\
2M05414512-0154470 & 2M05414512-0154470 & 05:41:45.126 & -01:54:47.19 & -99.00 & -99.00 & Unclassified & 386.4 & 400.0\\
HOPS-384-C & HOPS-384 & 05:41:44.252 & -01:54:55.53 & 1404.97 & 51.90 & 0 & 527.0 & 409.5\\
HOPS-384-region-E & HOPS-384 & 05:41:45.735 & -01:54:57.97 & 1404.97 & 51.90 & 0 & 386.4 & 409.5\\
2M05414418-0155203 & 2M05414418-0155203 & 05:41:44.184 & -01:55:20.52 & -99.00 & -99.00 & Unclassified & 266.0 & 400.0\\
HOPS-304-A & HOPS-304 & 05:41:45.954 & -01:56:26.59 & 4.03 & 354.90 & Flat & 153.3 & 409.5\\
HOPS-304-B & HOPS-304 & 05:41:45.912 & -01:56:26.80 & 4.03 & 354.90 & Flat & 153.3 & 409.5\\
HOPS-303 & HOPS-303 & 05:42:02.649 & -02:07:45.98 & 1.42 & 43.20 & 0 & 3.4 & 410.0\\
HOPS-299 & HOPS-299 & 05:41:44.610 & -02:16:06.63 & 18.62 & 277.00 & I & 45.9 & 408.7\\
HOPS-300 & HOPS-300 & 05:41:24.212 & -02:16:06.66 & 0.72 & 93.70 & I & 24.9 & 407.9\\
HOPS-298-A & HOPS-298 & 05:41:37.192 & -02:17:17.35 & 29.42 & 169.30 & I & 48.2 & 408.4\\
HOPS-298-B & HOPS-298 & 05:41:37.040 & -02:17:18.01 & 29.42 & 169.30 & I & 48.2 & 408.4\\
HOPS-297 & HOPS-297 & 05:41:23.294 & -02:17:35.79 & 0.19 & 274.90 & I & 26.0 & 407.8\\
HOPS-399 & HOPS-399 & 05:41:24.932 & -02:18:06.68 & 5.98 & 31.10 & 0 & 32.7 & 407.9\\
HOPS-372 & HOPS-372 & 05:41:26.370 & -02:18:20.18 & 4.53 & 37.30 & 0 & 40.3 & 407.9\\
HOPS-398 & HOPS-398 & 05:41:29.414 & -02:21:16.42 & 0.95 & 23.00 & 0 & 12.6 & 408.0\\
HOPS-295 & HOPS-295 & 05:41:28.961 & -02:23:19.56 & 0.30 & 86.60 & I & 6.0 & 407.9\\
HOPS-294 & HOPS-294 & 05:40:51.733 & -02:26:49.02 & 2.62 & 606.80 & Flat & 2.2 & 406.4\\
HOPS-107 & HOPS-107 & 05:35:23.353 & -04:40:10.29 & 4.43 & 472.00 & Flat & 29.3 & 392.7\\
HOPS-105 & HOPS-105 & 05:35:32.299 & -04:46:48.44 & 0.10 & 520.30 & Flat & 42.7 & 392.6\\
HOPS-102 & HOPS-102 & 05:34:35.168 & -04:52:17.96 & 0.47 & 479.20 & I & 26.8 & 392.3\\
HOPS-99 & HOPS-99 & 05:34:29.468 & -04:55:30.25 & 1.16 & 48.90 & 0 & 18.2 & 392.1\\
HOPS-96 & HOPS-96 & 05:35:29.718 & -04:58:48.60 & 5.41 & 35.60 & 0 & 89.6 & 392.7\\
V2273Ori & V2273Ori & 05:35:15.602 & -04:59:27.96 & -99.00 & -99.00 & Unclassified & 69.6 & 392.7\\
HOPS-383 & HOPS-383 & 05:35:29.785 & -04:59:50.41 & 6.85 & 45.80 & 0 & 51.8 & 392.8\\
HOPS-95 & HOPS-95 & 05:35:34.205 & -04:59:52.41 & 0.68 & 41.80 & 0 & 56.7 & 392.8\\
HOPS-94 & HOPS-94 & 05:35:16.167 & -05:00:02.51 & 5.73 & 123.00 & I & 67.3 & 392.7\\
HOPS-93 & HOPS-93 & 05:35:15.048 & -05:00:08.05 & 0.37 & 107.30 & I & 67.3 & 392.7\\
J05351805-050017.98 & J05351805-050017.98 & 05:35:18.051 & -05:00:17.98 & -99.00 & -99.00 & Unclassified & 192.8 & 392.7\\
HOPS-92-A-A & HOPS-92 & 05:35:18.337 & -05:00:32.94 & 17.58 & 186.30 & Flat & 139.2 & 392.7\\
HOPS-92-A-B & HOPS-92 & 05:35:18.328 & -05:00:33.18 & 17.58 & 186.30 & Flat & 139.2 & 392.7\\
HOPS-92-B & HOPS-92 & 05:35:18.270 & -05:00:33.92 & 17.58 & 186.30 & Flat & 139.2 & 392.7\\
HOPS-91 & HOPS-91 & 05:35:18.925 & -05:00:51.11 & 3.62 & 41.70 & 0 & 146.8 & 392.7\\
HOPS-90 & HOPS-90 & 05:35:34.492 & -05:00:52.34 & 2.43 & 417.70 & Flat & 60.2 & 392.8\\
HOPS-89 & HOPS-89 & 05:35:19.975 & -05:01:02.56 & 1.38 & 158.30 & Flat & 166.1 & 392.7\\
HOPS-88 & HOPS-88 & 05:35:22.471 & -05:01:14.31 & 13.82 & 42.40 & 0 & 139.2 & 392.7\\
HOPS-87 & HOPS-87 & 05:35:23.420 & -05:01:30.54 & 31.90 & 38.10 & 0 & 125.6 & 392.7\\
HOPS-86-A & HOPS-86 & 05:35:23.654 & -05:01:40.26 & 2.86 & 112.70 & I & 108.0 & 392.7\\
HOPS-86-B & HOPS-86 & 05:35:23.733 & -05:01:48.13 & 2.86 & 112.70 & I & 108.0 & 392.7\\
HOPS-85-A & HOPS-85 & 05:35:28.189 & -05:03:41.20 & 14.24 & 174.20 & Flat & 77.4 & 392.8\\
HOPS-85-B & HOPS-85 & 05:35:28.193 & -05:03:41.29 & 14.24 & 174.20 & Flat & 77.4 & 392.8\\
HOPS-84-A & HOPS-84 & 05:35:26.560 & -05:03:55.12 & 42.96 & 90.80 & I & 71.7 & 392.8\\
HOPS-84-B & HOPS-84 & 05:35:26.537 & -05:03:55.73 & 42.96 & 90.80 & I & 71.7 & 392.8\\
HOPS-82 & HOPS-82 & 05:35:19.740 & -05:04:54.50 & 2.10 & 116.40 & Flat & 55.0 & 392.7\\
HOPS-81 & HOPS-81 & 05:35:28.019 & -05:04:57.35 & 1.08 & 40.10 & 0 & 188.9 & 392.8\\
HOPS-80 & HOPS-80 & 05:35:25.183 & -05:05:09.37 & 0.07 & 275.30 & Flat & 146.5 & 392.8\\
HOPS-78-A & HOPS-78 & 05:35:25.966 & -05:05:43.33 & 7.81 & 38.10 & 0 & 157.8 & 392.8\\
HOPS-78-E & HOPS-78 & 05:35:25.763 & -05:05:43.83 & 8.10 & 38.10 & 0 & 157.8 & 400.0\\
HOPS-78-B & HOPS-78 & 05:35:26.148 & -05:05:45.80 & 7.81 & 38.10 & 0 & 157.8 & 392.8\\
HOPS-77-B & HOPS-77 & 05:35:31.470 & -05:05:46.10 & 11.26 & 550.30 & Flat & 104.5 & 392.8\\
HOPS-78-C & HOPS-78 & 05:35:26.181 & -05:05:47.12 & 7.81 & 38.10 & 0 & 157.8 & 392.8\\
HOPS-77-A-A & HOPS-77 & 05:35:31.539 & -05:05:47.33 & 11.26 & 550.30 & Flat & 104.5 & 392.8\\
HOPS-77-A-B & HOPS-77 & 05:35:31.545 & -05:05:47.40 & 11.26 & 550.30 & Flat & 104.5 & 392.8\\
HOPS-78-D & HOPS-78 & 05:35:25.920 & -05:05:47.70 & 7.81 & 38.10 & 0 & 157.8 & 392.8\\
HOPS-76 & HOPS-76 & 05:35:25.763 & -05:05:58.13 & 1.62 & 135.50 & I & 180.3 & 392.8\\
HOPS-75-A & HOPS-75 & 05:35:26.680 & -05:06:10.51 & 3.52 & 67.90 & 0 & 248.0 & 392.8\\
HOPS-75-B & HOPS-75 & 05:35:26.678 & -05:06:10.76 & 3.52 & 67.90 & 0 & 248.0 & 392.8\\
HOPS-74 & HOPS-74 & 05:35:24.874 & -05:06:21.58 & 1.00 & 516.50 & Flat & 187.4 & 392.8\\
HOPS-73 & HOPS-73 & 05:35:27.699 & -05:07:04.32 & 1.48 & 43.00 & 0 & 177.0 & 392.8\\
HOPS-72 & HOPS-72 & 05:35:25.724 & -05:07:46.24 & 0.48 & 693.00 & Unclassified & 304.2 & 392.8\\
HOPS-394-A & HOPS-394 & 05:35:24.046 & -05:07:52.11 & 5.74 & 45.50 & 0 & 370.5 & 392.8\\
HOPS-394-B & HOPS-394 & 05:35:24.867 & -05:07:54.64 & 5.74 & 45.50 & 0 & 326.1 & 392.8\\
HOPS-71-B & HOPS-71 & 05:35:25.541 & -05:07:56.84 & 4.90 & 277.50 & I & 326.1 & 392.8\\
HOPS-71-A & HOPS-71 & 05:35:25.582 & -05:07:57.64 & 4.90 & 277.50 & I & 326.1 & 392.8\\
HOPS-70-B-B & HOPS-70 & 05:35:22.570 & -05:08:00.32 & 6.04 & 619.30 & Flat & 318.0 & 392.8\\
HOPS-70-B-A & HOPS-70 & 05:35:22.562 & -05:08:00.72 & 6.04 & 619.30 & Flat & 318.0 & 392.8\\
HOPS-70-C & HOPS-70 & 05:35:21.938 & -05:08:04.58 & 6.04 & 619.30 & Flat & 318.0 & 392.8\\
HOPS-70-A-B & HOPS-70 & 05:35:22.426 & -05:08:05.03 & 6.04 & 619.30 & Flat & 318.0 & 392.8\\
HOPS-70-A-A & HOPS-70 & 05:35:22.406 & -05:08:05.14 & 6.04 & 619.30 & Flat & 318.0 & 392.8\\
HOPS-68 & HOPS-68 & 05:35:24.299 & -05:08:30.74 & 4.96 & 100.60 & I & 469.7 & 392.8\\
HOPS-66-B & HOPS-66 & 05:35:26.927 & -05:09:22.43 & 18.33 & 264.90 & Flat & 345.9 & 392.8\\
HOPS-66-A & HOPS-66 & 05:35:26.857 & -05:09:24.40 & 18.33 & 264.90 & Flat & 345.9 & 392.8\\
HOPS-370 & HOPS-370 & 05:35:27.634 & -05:09:34.42 & 315.63 & 71.50 & I & 380.4 & 392.8\\
HOPS-65 & HOPS-65 & 05:35:21.576 & -05:09:38.85 & 0.31 & 545.70 & I & 170.5 & 392.8\\
2MJ05352746-0509441 & 2MJ05352746-0509441 & 05:35:27.472 & -05:09:44.14 & -99.00 & -99.00 & Unclassified & 426.9 & 400.0\\
HOPS-64 & HOPS-64 & 05:35:26.998 & -05:09:54.08 & 13.42 & 29.70 & I & 738.4 & 392.8\\
HOPS-108 & HOPS-108 & 05:35:27.086 & -05:10:00.06 & 33.52 & 38.50 & 0 & 589.4 & 392.8\\
VLA16 & HOPS-108 & 05:35:26.824 & -05:10:05.62 & -99.00 & -99.00 & 0 & 1258.8 & 392.8\\
VLA15 & HOPS-108 & 05:35:26.410 & -05:10:05.94 & -99.00 & -99.00 & 0 & 1258.8 & 392.8\\
OMC2-FIR4-ALMA1 & OMC2-FIR4-ALMA1 & 05:35:26.785 & -05:10:08.83 & -99.00 & -99.00 & Unclassified & 834.0 & 392.8\\
HOPS-369 & HOPS-369 & 05:35:26.969 & -05:10:17.27 & 30.89 & 379.20 & Flat & 380.4 & 392.8\\
HOPS-368 & HOPS-368 & 05:35:24.725 & -05:10:30.08 & 60.22 & 137.50 & I & 199.8 & 392.8\\
HOPS-60 & HOPS-60 & 05:35:23.287 & -05:12:03.41 & 19.18 & 54.10 & 0 & 95.3 & 392.8\\
2MJ05352131-0512126 & 2MJ05352131-0512126 & 05:35:21.318 & -05:12:12.68 & -99.00 & -99.00 & Unclassified & 208.5 & 400.0\\
HOPS-59-B & HOPS-59 & 05:35:20.134 & -05:13:13.31 & 43.25 & 528.40 & Flat & 331.7 & 392.8\\
HOPS-59-A & HOPS-59 & 05:35:20.151 & -05:13:15.70 & 43.25 & 528.40 & Flat & 331.7 & 392.8\\
HOPS-409 & HOPS-409 & 05:35:21.363 & -05:13:17.83 & 7.15 & 28.40 & 0 & 314.9 & 392.8\\
HOPS-58 & HOPS-58 & 05:35:18.523 & -05:13:38.34 & 3.94 & 620.00 & Flat & 274.1 & 392.8\\
HOPS-57-A & HOPS-57 & 05:35:19.887 & -05:15:08.18 & 2.82 & 421.20 & Flat & 295.7 & 392.8\\
HOPS-57-B & HOPS-57 & 05:35:19.833 & -05:15:09.03 & 2.82 & 421.20 & Flat & 295.7 & 392.8\\
HOPS-56-A-C & HOPS-56 & 05:35:19.481 & -05:15:32.81 & 20.40 & 48.10 & 0 & 338.5 & 392.8\\
V1334Ori & V1334Ori & 05:35:17.923 & -05:15:32.84 & -99.00 & -99.00 & Unclassified & 427.9 & 392.8\\
HOPS-56-A-B & HOPS-56 & 05:35:19.470 & -05:15:32.96 & 20.40 & 48.10 & 0 & 338.5 & 392.8\\
HOPS-56-A-A & HOPS-56 & 05:35:19.482 & -05:15:33.08 & 20.40 & 48.10 & 0 & 338.5 & 392.8\\
V2358Ori & V2358Ori & 05:35:19.811 & -05:15:35.20 & -99.00 & -99.00 & Unclassified & 340.1 & 392.8\\
HOPS-56-B & HOPS-56 & 05:35:19.420 & -05:15:38.29 & 20.40 & 48.10 & 0 & 338.5 & 392.8\\
J05352074-0515492 & J05352074-0515492 & 05:35:20.751 & -05:15:49.26 & -99.00 & -99.00 & Unclassified & 679.9 & 392.8\\
OMC1N-1-A & OMC1N-1-A & 05:35:17.890 & -05:18:35.41 & -99.00 & -99.00 & Unclassified & 273.6 & 392.8\\
OMC1N-1-B & OMC1N-1-B & 05:35:16.812 & -05:19:01.00 & -99.00 & -99.00 & Unclassified & 300.6 & 392.8\\
OMC1N-1-C & OMC1N-1-C & 05:35:17.145 & -05:19:12.70 & -99.00 & -99.00 & Unclassified & 836.1 & 392.8\\
OMC1N-2-3 & OMC1N-2-3 & 05:35:16.611 & -05:19:35.69 & -99.00 & -99.00 & Unclassified & 271.6 & 392.8\\
OMC1N-4-5-A & OMC1N-4-5-A & 05:35:16.040 & -05:19:44.61 & -99.00 & -99.00 & Unclassified & 707.3 & 392.8\\
OMC1N-4-5-B & OMC1N-4-5-B & 05:35:16.047 & -05:20:05.61 & -99.00 & -99.00 & Unclassified & 707.3 & 392.8\\
OMC1N-4-5-C & OMC1N-4-5-C & 05:35:15.973 & -05:20:14.25 & -99.00 & -99.00 & Unclassified & 1852.9 & 392.8\\
OMC1N-6-7-8-A-A & OMC1N-6-7-8-A-A & 05:35:18.673 & -05:20:33.71 & -99.00 & -99.00 & Unclassified & 2788.1 & 392.8\\
OMC1N-6-7-8-A-B & OMC1N-6-7-8-A-B & 05:35:18.660 & -05:20:33.82 & -99.00 & -99.00 & Unclassified & 2788.1 & 392.8\\
OMC1N-6-7-8-E & OMC1N-6-7-8-E & 05:35:15.698 & -05:20:39.32 & -99.00 & -99.00 & Unclassified & 2387.3 & 392.8\\
OMC1N-6-7-8-D & OMC1N-6-7-8-D & 05:35:16.659 & -05:20:44.44 & -99.00 & -99.00 & Unclassified & 1852.9 & 392.8\\
OMC1N-6-7-8-B & OMC1N-6-7-8-B & 05:35:18.192 & -05:20:48.46 & -99.00 & -99.00 & Unclassified & 2788.1 & 392.8\\
OMC1N-6-7-8-C & OMC1N-6-7-8-C & 05:35:18.001 & -05:20:55.76 & -99.00 & -99.00 & Unclassified & 2387.3 & 392.8\\
OMC1N-6-7-8-F & OMC1N-6-7-8-F & 05:35:16.278 & -05:21:09.13 & -99.00 & -99.00 & Unclassified & 418.6 & 392.8\\
OMC1N-6-7-8-G & OMC1N-6-7-8-G & 05:35:15.402 & -05:21:13.98 & -99.00 & -99.00 & Unclassified & 421.1 & 392.8\\
OMC1N-6-7-8-H & OMC1N-6-7-8-H & 05:35:15.604 & -05:21:26.88 & -99.00 & -99.00 & Unclassified & 1688.7 & 392.8\\
HOPS-53 & HOPS-53 & 05:33:57.395 & -05:23:29.99 & 22.84 & 45.90 & 0 & 11.8 & 390.5\\
HOPS-50 & HOPS-50 & 05:34:40.914 & -05:31:44.71 & 3.65 & 51.40 & 0 & 38.6 & 391.5\\
HOPS-49 & HOPS-49 & 05:34:48.885 & -05:31:45.79 & 0.62 & 356.80 & I & 43.0 & 391.8\\
HOPS-47 & HOPS-47 & 05:33:45.882 & -05:32:58.12 & 0.10 & 558.40 & Flat & 9.4 & 389.8\\
HOPS-45-A & HOPS-45 & 05:35:06.457 & -05:33:34.98 & 7.40 & 517.80 & Flat & 65.7 & 391.9\\
HOPS-45-B & HOPS-45 & 05:35:06.454 & -05:33:35.28 & 7.40 & 517.80 & Flat & 65.7 & 391.9\\
HOPS-44 & HOPS-44 & 05:35:10.591 & -05:35:06.26 & 1.52 & 43.80 & 0 & 95.0 & 391.8\\
HOPS-43 & HOPS-43 & 05:35:04.503 & -05:35:14.78 & 2.84 & 75.00 & I & 69.0 & 391.7\\
HOPS-42 & HOPS-42 & 05:35:05.061 & -05:35:40.79 & 0.24 & 200.90 & I & 90.6 & 391.7\\
HOPS-41 & HOPS-41 & 05:34:29.463 & -05:35:42.80 & 1.68 & 82.30 & I & 23.0 & 390.9\\
HOPS-40 & HOPS-40 & 05:35:08.440 & -05:35:58.57 & 2.34 & 38.10 & 0 & 96.5 & 391.6\\
HOPS-36 & HOPS-36 & 05:34:26.453 & -05:37:40.75 & 0.89 & 374.60 & Flat & 19.9 & 390.6\\
HOPS-32-A & HOPS-32 & 05:34:35.454 & -05:39:59.33 & 1.74 & 58.90 & 0 & 26.1 & 390.6\\
HOPS-32-B & HOPS-32 & 05:34:35.432 & -05:39:59.58 & 1.74 & 58.90 & 0 & 26.1 & 390.6\\
HOPS-30 & HOPS-30 & 05:34:44.055 & -05:41:25.84 & 3.28 & 81.20 & I & 55.1 & 390.6\\
HOPS-29 & HOPS-29 & 05:34:49.043 & -05:41:42.40 & 1.66 & 148.20 & I & 83.2 & 390.6\\
HOPS-28-A & HOPS-28 & 05:34:47.320 & -05:41:56.08 & 0.43 & 46.30 & 0 & 62.7 & 390.6\\
HOPS-28-B & HOPS-28 & 05:34:47.303 & -05:41:56.29 & 0.43 & 46.30 & 0 & 62.7 & 390.6\\
HOPS-20-B & HOPS-20 & 05:33:30.712 & -05:50:41.26 & 1.06 & 94.80 & I & 2.1 & 389.1\\
HOPS-20-A & HOPS-20 & 05:33:30.704 & -05:50:41.29 & 1.06 & 94.80 & I & 2.1 & 389.1\\
HOPS-18 & HOPS-18 & 05:35:05.515 & -05:51:54.42 & 1.22 & 71.80 & I & 36.1 & 389.2\\
HOPS-17 & HOPS-17 & 05:35:07.185 & -05:52:06.07 & 0.26 & 341.30 & I & 36.8 & 389.1\\
HOPS-15 & HOPS-15 & 05:36:19.027 & -05:55:25.40 & 0.15 & 342.00 & Flat & 6.9 & 388.6\\
HOPS-16 & HOPS-16 & 05:35:00.822 & -05:55:26.07 & 0.58 & 361.00 & Flat & 37.6 & 388.6\\
HOPS-13 & HOPS-13 & 05:35:24.581 & -05:55:33.74 & 0.98 & 383.60 & Flat & 20.5 & 388.7\\
HOPS-371 & HOPS-371 & 05:35:10.419 & -05:55:40.55 & 0.49 & 31.60 & 0 & 39.7 & 388.6\\
HOPS-12-A & HOPS-12 & 05:35:08.631 & -05:55:54.64 & 6.26 & 42.00 & 0 & 49.8 & 388.6\\
HOPS-12-B-B & HOPS-12 & 05:35:08.955 & -05:55:54.88 & 6.26 & 42.00 & 0 & 49.8 & 388.6\\
HOPS-12-B-A & HOPS-12 & 05:35:08.945 & -05:55:55.03 & 6.26 & 42.00 & 0 & 49.8 & 388.6\\
HOPS-11 & HOPS-11 & 05:35:13.424 & -05:57:57.88 & 7.69 & 48.80 & 0 & 36.9 & 388.3\\
HOPS-10 & HOPS-10 & 05:35:09.050 & -05:58:26.87 & 2.84 & 46.20 & 0 & 32.4 & 388.2\\
HOPS-192 & HOPS-192 & 05:36:32.472 & -06:01:16.45 & 1.20 & 202.50 & Flat & 4.8 & 387.8\\
HOPS-193-A & HOPS-193 & 05:36:30.282 & -06:01:17.11 & 0.98 & 226.70 & I & 5.2 & 387.8\\
HOPS-193-B & HOPS-193 & 05:36:30.283 & -06:01:17.37 & 0.98 & 226.70 & I & 5.2 & 387.8\\
HOPS-200 & HOPS-200 & 05:35:33.214 & -06:06:09.62 & 0.24 & 244.40 & Flat & 12.0 & 387.1\\
HOPS-194 & HOPS-194 & 05:35:52.027 & -06:10:01.67 & 10.77 & 645.00 & Flat & 14.2 & 386.6\\
HOPS-191 & HOPS-191 & 05:36:17.273 & -06:11:11.21 & 0.49 & 196.70 & I & 6.9 & 386.6\\
HOPS-198 & HOPS-198 & 05:35:22.196 & -06:13:06.14 & 0.72 & 61.40 & 0 & 11.6 & 386.0\\
HOPS-185 & HOPS-185 & 05:36:36.969 & -06:14:58.78 & 0.88 & 96.90 & I & 6.3 & 386.1\\
HOPS-181-B & HOPS-181 & 05:36:19.655 & -06:22:08.95 & 5.22 & 131.30 & I & 353.8 & 385.1\\
HOPS-182-A & HOPS-182 & 05:36:18.795 & -06:22:10.21 & 59.79 & 51.90 & 0 & 409.5 & 385.1\\
HOPS-182-B & HOPS-182 & 05:36:18.775 & -06:22:11.15 & 59.79 & 51.90 & 0 & 409.5 & 385.1\\
HOPS-181-A & HOPS-181 & 05:36:19.504 & -06:22:11.99 & 5.22 & 131.30 & I & 353.8 & 385.1\\
HOPS-182-C & HOPS-182 & 05:36:18.478 & -06:22:13.62 & 59.79 & 51.90 & 0 & 409.5 & 385.1\\
HOPS-183-B & HOPS-183 & 05:36:17.912 & -06:22:27.25 & 0.25 & 224.50 & Flat & 221.4 & 385.1\\
HOPS-183-A & HOPS-183 & 05:36:17.873 & -06:22:27.91 & 0.25 & 224.50 & Flat & 221.4 & 385.1\\
HOPS-178 & HOPS-178 & 05:36:24.622 & -06:22:41.14 & 16.84 & 155.10 & I & 179.1 & 385.1\\
HOPS-179 & HOPS-179 & 05:36:21.876 & -06:23:29.91 & 1.55 & 467.50 & Flat & 140.2 & 385.0\\
HOPS-176 & HOPS-176 & 05:36:23.603 & -06:24:51.48 & 1.28 & 312.20 & Flat & 124.6 & 384.9\\
HOPS-174 & HOPS-174 & 05:36:25.868 & -06:24:58.67 & 1.67 & 350.30 & Flat & 94.3 & 384.9\\
HOPS-173-A & HOPS-173 & 05:36:26.041 & -06:25:05.09 & 0.79 & 60.20 & 0 & 83.7 & 384.9\\
HOPS-173-B & HOPS-173 & 05:36:26.051 & -06:25:05.31 & 0.79 & 60.20 & 0 & 83.7 & 384.9\\
HOPS-199 & HOPS-199 & 05:34:39.887 & -06:25:14.02 & 0.15 & 576.70 & Flat & 4.4 & 385.3\\
HOPS-186 & HOPS-186 & 05:35:47.306 & -06:26:14.71 & 0.41 & 72.30 & I & 15.1 & 384.3\\
HOPS-189 & HOPS-189 & 05:35:30.921 & -06:26:32.00 & 1.04 & 133.10 & I & 14.9 & 384.3\\
HOPS-188 & HOPS-188 & 05:35:29.844 & -06:26:58.13 & 15.74 & 103.30 & I & 13.8 & 384.2\\
HOPS-172 & HOPS-172 & 05:36:19.463 & -06:29:06.91 & 0.55 & 149.80 & I & 11.2 & 384.4\\
HOPS-170-B & HOPS-170 & 05:36:41.322 & -06:33:59.26 & 2.11 & 832.50 & Flat & 8.7 & 384.2\\
HOPS-170-A & HOPS-170 & 05:36:41.368 & -06:34:00.75 & 2.11 & 832.50 & Flat & 8.7 & 384.2\\
HOPS-197 & HOPS-197 & 05:34:15.897 & -06:34:32.66 & 0.17 & 506.60 & Flat & 7.2 & 385.1\\
HOPS-177 & HOPS-177 & 05:35:50.017 & -06:34:53.47 & 0.35 & 84.70 & I & 5.4 & 383.6\\
HOPS-163-B & HOPS-163 & 05:37:17.329 & -06:36:18.10 & 0.76 & 432.30 & I & 4.4 & 385.7\\
HOPS-163-A & HOPS-163 & 05:37:17.277 & -06:36:18.19 & 0.76 & 432.30 & I & 4.4 & 385.7\\
HOPS-164 & HOPS-164 & 05:37:00.425 & -06:37:10.89 & 0.49 & 50.00 & 0 & 7.3 & 385.0\\
HOPS-171 & HOPS-171 & 05:36:17.208 & -06:38:01.51 & 1.54 & 61.80 & 0 & 7.4 & 383.4\\
HOPS-169 & HOPS-169 & 05:36:36.160 & -06:38:54.35 & 3.27 & 32.50 & 0 & 7.9 & 384.0\\
HOPS-166 & HOPS-166 & 05:36:25.131 & -06:44:41.83 & 12.89 & 457.10 & Flat & 55.4 & 383.5\\
HOPS-168-B & HOPS-168 & 05:36:18.952 & -06:45:23.48 & 40.03 & 54.00 & 0 & 25.0 & 383.3\\
HOPS-168-A & HOPS-168 & 05:36:18.941 & -06:45:23.58 & 40.03 & 54.00 & 0 & 25.0 & 383.3\\
HOPS-167 & HOPS-167 & 05:36:19.808 & -06:46:00.82 & 0.15 & 568.60 & Flat & 18.7 & 383.3\\
HOPS-203-A & HOPS-203 & 05:36:22.865 & -06:46:06.63 & 17.04 & 43.70 & 0 & 23.3 & 383.5\\
HOPS-203-B & HOPS-203 & 05:36:22.862 & -06:46:06.75 & 17.04 & 43.70 & 0 & 23.3 & 383.5\\
HOPS-203-C & HOPS-203 & 05:36:22.898 & -06:46:09.47 & 17.04 & 43.70 & 0 & 23.3 & 383.5\\
HOPS-165 & HOPS-165 & 05:36:23.539 & -06:46:14.52 & 2.84 & 96.10 & I & 24.4 & 383.5\\
HOPS-159 & HOPS-159 & 05:37:53.764 & -06:47:17.07 & 0.38 & 498.40 & Flat & 10.6 & 387.4\\
HOPS-160 & HOPS-160 & 05:37:51.056 & -06:47:20.64 & 1.16 & 80.40 & I & 8.7 & 387.3\\
HOPS-355 & HOPS-355 & 05:37:17.123 & -06:49:49.12 & 0.99 & 44.90 & 0 & 3.0 & 385.8\\
HOPS-157 & HOPS-157 & 05:37:56.574 & -06:56:39.47 & 3.26 & 77.60 & I & 12.4 & 387.7\\
HOPS-156 & HOPS-156 & 05:38:03.430 & -06:58:15.89 & 0.23 & 90.10 & I & 13.9 & 388.1\\
HOPS-149-B & HOPS-149 & 05:38:40.472 & -06:58:19.22 & 9.88 & 484.60 & Flat & 108.8 & 389.9\\
HOPS-149-A & HOPS-149 & 05:38:40.496 & -06:58:21.99 & 9.88 & 484.60 & Flat & 108.8 & 389.9\\
HOPS-158-A & HOPS-158 & 05:37:24.473 & -06:58:32.90 & 2.26 & 591.60 & Flat & 4.9 & 386.2\\
HOPS-158-B & HOPS-158 & 05:37:24.480 & -06:58:32.95 & 2.26 & 591.60 & Flat & 4.9 & 386.2\\
HOPS-154 & HOPS-154 & 05:38:20.113 & -06:59:04.78 & 0.09 & 166.70 & I & 9.0 & 388.9\\
HOPS-148 & HOPS-148 & 05:38:39.523 & -06:59:30.23 & 0.36 & 262.90 & I & 78.4 & 389.9\\
HOPS-143 & HOPS-143 & 05:38:46.193 & -07:00:48.47 & 3.70 & 242.10 & I & 414.7 & 390.3\\
HOPS-144 & HOPS-144 & 05:38:45.024 & -07:01:01.69 & 1.86 & 99.20 & I & 261.8 & 390.2\\
HOPS-377 & HOPS-377 & 05:38:45.536 & -07:01:01.98 & 3.31 & 53.70 & 0 & 323.7 & 390.2\\
HOPS-145-B & HOPS-145 & 05:38:43.203 & -07:01:07.39 & 1.80 & 133.70 & I & 258.0 & 390.2\\
HOPS-145-A & HOPS-145 & 05:38:43.851 & -07:01:13.10 & 1.80 & 133.70 & I & 258.0 & 390.2\\
HOPS-139 & HOPS-139 & 05:38:49.626 & -07:01:17.63 & 2.49 & 84.30 & I & 193.0 & 390.5\\
HOPS-140-C & HOPS-140 & 05:38:46.282 & -07:01:51.38 & 0.51 & 137.20 & I & 222.2 & 390.3\\
HOPS-140-B & HOPS-140 & 05:38:46.274 & -07:01:53.62 & 0.51 & 137.20 & I & 222.2 & 390.3\\
HOPS-140-A & HOPS-140 & 05:38:45.717 & -07:01:58.54 & 0.51 & 137.20 & I & 222.2 & 390.3\\
HOPS-376 & HOPS-376 & 05:38:18.099 & -07:02:25.95 & 186.71 & 492.00 & Flat & 6.9 & 388.8\\
HOPS-138-A & HOPS-138 & 05:38:48.317 & -07:02:43.68 & 0.10 & 42.80 & 0 & 167.9 & 390.5\\
HOPS-138-B & HOPS-138 & 05:38:48.338 & -07:02:43.68 & 0.10 & 42.80 & 0 & 167.9 & 390.5\\
HOPS-136 & HOPS-136 & 05:38:46.529 & -07:05:37.41 & 0.60 & 161.70 & I & 32.6 & 390.6\\
HOPS-153 & HOPS-153 & 05:37:57.023 & -07:06:56.27 & 3.78 & 39.40 & 0 & 6.4 & 387.9\\
HOPS-152 & HOPS-152 & 05:37:58.748 & -07:07:25.73 & 0.60 & 53.80 & 0 & 6.7 & 388.0\\
HOPS-150-A & HOPS-150 & 05:38:07.530 & -07:08:29.01 & 3.22 & 245.20 & Flat & 6.2 & 388.5\\
HOPS-150-B & HOPS-150 & 05:38:07.530 & -07:08:32.23 & 3.22 & 245.20 & Flat & 6.2 & 388.5\\
HOPS-129 & HOPS-129 & 05:39:11.868 & -07:10:34.88 & 1.47 & 191.30 & Flat & 8.0 & 393.8\\
HOPS-133 & HOPS-133 & 05:39:05.834 & -07:10:39.24 & 2.89 & 74.60 & I & 10.9 & 393.1\\
HOPS-131 & HOPS-131 & 05:39:07.579 & -07:10:52.22 & 0.14 & 82.30 & I & 9.0 & 393.4\\
HOPS-135 & HOPS-135 & 05:38:45.328 & -07:10:56.04 & 0.99 & 130.30 & I & 9.2 & 391.1\\
HOPS-132 & HOPS-132 & 05:39:05.371 & -07:11:05.17 & 1.49 & 616.30 & Flat & 9.4 & 393.2\\
HOPS-134 & HOPS-134 & 05:38:42.791 & -07:12:43.82 & 6.74 & 781.90 & Flat & 6.2 & 391.2\\
HOPS-130 & HOPS-130 & 05:39:02.979 & -07:12:52.20 & 1.29 & 156.70 & I & 10.4 & 393.2\\
HOPS-122 & HOPS-122 & 05:39:45.139 & -07:19:13.43 & 0.02 & 246.00 & I & 11.4 & 400.1\\
HOPS-127 & HOPS-127 & 05:39:00.972 & -07:20:22.55 & 0.35 & 133.30 & I & 6.5 & 394.5\\
HOPS-128-A & HOPS-128 & 05:38:52.015 & -07:21:05.87 & 0.71 & 469.20 & Flat & 4.9 & 393.6\\
HOPS-128-B & HOPS-128 & 05:38:52.378 & -07:21:09.32 & 0.71 & 469.20 & Flat & 4.9 & 393.6\\
HOPS-123 & HOPS-123 & 05:39:33.286 & -07:22:57.45 & 0.37 & 50.10 & 0 & 25.9 & 399.0\\
HOPS-119 & HOPS-119 & 05:39:50.689 & -07:23:30.58 & 0.97 & 573.80 & Flat & 26.9 & 402.3\\
HOPS-408 & HOPS-408 & 05:39:30.904 & -07:23:59.67 & 0.47 & 37.90 & 0 & 32.0 & 398.9\\
HOPS-118 & HOPS-118 & 05:39:54.605 & -07:24:14.97 & 0.26 & 552.80 & Flat & 35.1 & 403.4\\
HOPS-117 & HOPS-117 & 05:39:55.460 & -07:24:19.48 & 0.10 & 277.00 & Flat & 35.1 & 403.6\\
HOPS-395-A & HOPS-395 & 05:39:17.092 & -07:24:24.55 & 0.44 & 31.70 & 0 & 22.4 & 397.2\\
HOPS-395-B & HOPS-395 & 05:39:17.081 & -07:24:24.57 & 0.44 & 31.70 & 0 & 22.4 & 397.2\\
HOPS-116 & HOPS-116 & 05:39:57.912 & -07:25:13.09 & 0.27 & 411.10 & Flat & 35.5 & 404.4\\
HOPS-114 & HOPS-114 & 05:40:01.391 & -07:25:38.76 & 0.04 & 117.30 & I & 47.8 & 405.3\\
HOPS-115 & HOPS-115 & 05:39:56.542 & -07:25:51.62 & 0.29 & 461.30 & Flat & 57.0 & 404.2\\
HOPS-124 & HOPS-124 & 05:39:19.911 & -07:26:11.23 & 52.35 & 44.80 & 0 & 26.3 & 398.0\\
HOPS-120 & HOPS-120 & 05:39:34.324 & -07:26:11.29 & 0.29 & 455.30 & Flat & 22.9 & 400.0\\
HOPS-125 & HOPS-125 & 05:39:19.540 & -07:26:17.13 & 8.60 & 110.50 & Flat & 23.7 & 398.0\\
HOPS-287 & HOPS-287 & 05:40:08.789 & -07:27:27.91 & 0.71 & 117.80 & I & 22.3 & 407.6\\
HOPS-291 & HOPS-291 & 05:39:57.954 & -07:28:57.62 & 0.09 & 340.10 & Flat & 49.8 & 405.5\\
HOPS-290-B & HOPS-290 & 05:39:57.329 & -07:29:32.71 & 1.72 & 47.30 & 0 & 73.8 & 405.5\\
HOPS-290-A & HOPS-290 & 05:39:57.377 & -07:29:33.10 & 1.72 & 47.30 & 0 & 73.8 & 405.5\\
HOPS-288-A-A & HOPS-288 & 05:39:56.001 & -07:30:27.57 & 126.28 & 48.60 & 0 & 83.8 & 405.5\\
HOPS-288-A-B & HOPS-288 & 05:39:56.006 & -07:30:27.70 & 126.28 & 48.60 & 0 & 83.8 & 405.5\\
HOPS-288-B & HOPS-288 & 05:39:56.033 & -07:30:27.96 & 126.28 & 48.60 & 0 & 83.8 & 405.5\\
HOPS-282-A & HOPS-282 & 05:40:26.091 & -07:37:32.08 & 0.80 & 95.10 & I & 3.5 & 414.7\\
HOPS-282-B & HOPS-282 & 05:40:26.080 & -07:37:32.10 & 0.80 & 95.10 & I & 3.5 & 414.7\\
HOPS-281-A & HOPS-281 & 05:40:24.648 & -07:43:08.15 & 1.26 & 189.30 & Flat & 6.8 & 416.1\\
HOPS-281-B & HOPS-281 & 05:40:24.600 & -07:43:08.37 & 1.26 & 189.30 & Flat & 6.8 & 416.1\\
HOPS-276 & HOPS-276 & 05:40:42.924 & -07:45:01.98 & 0.15 & 303.80 & I & 10.5 & 421.0\\
HOPS-279 & HOPS-279 & 05:40:17.806 & -07:48:25.84 & 5.85 & 382.00 & Flat & 7.8 & 416.1\\
HOPS-280 & HOPS-280 & 05:40:14.953 & -07:48:48.64 & 3.22 & 121.20 & I & 6.1 & 415.5\\
HOPS-275 & HOPS-275 & 05:40:36.328 & -07:49:07.11 & 0.12 & 146.40 & I & 10.7 & 420.7\\
HOPS-267 & HOPS-267 & 05:41:19.675 & -07:50:41.03 & 1.10 & 186.20 & I & 21.9 & 428.9\\
HOPS-278 & HOPS-278 & 05:40:20.379 & -07:51:15.00 & 0.21 & 96.30 & I & 9.4 & 417.6\\
HOPS-265 & HOPS-265 & 05:41:20.350 & -07:53:10.71 & 0.14 & 635.10 & Flat & 48.6 & 429.5\\
HOPS-262 & HOPS-262 & 05:41:23.979 & -07:53:42.21 & 0.91 & 202.40 & Flat & 98.8 & 430.0\\
HOPS-263 & HOPS-263 & 05:41:23.691 & -07:53:46.76 & 0.75 & 145.10 & I & 114.2 & 430.0\\
HOPS-253 & HOPS-253 & 05:41:28.784 & -07:53:51.04 & 0.65 & 321.10 & Flat & 56.5 & 430.6\\
HOPS-258 & HOPS-258 & 05:41:24.727 & -07:54:08.51 & 1.12 & 385.70 & Flat & 115.1 & 430.2\\
HOPS-270 & HOPS-270 & 05:40:40.560 & -07:54:39.77 & 0.28 & 96.60 & I & 7.3 & 423.1\\
HOPS-274-A & HOPS-274 & 05:40:20.727 & -07:54:59.79 & 1.92 & 546.50 & Flat & 8.7 & 418.9\\
HOPS-274-B & HOPS-274 & 05:40:20.731 & -07:54:59.99 & 1.92 & 546.50 & Flat & 8.7 & 418.9\\
HOPS-254 & HOPS-254 & 05:41:24.518 & -07:55:07.41 & 6.24 & 114.70 & I & 87.0 & 430.4\\
HOPS-374 & HOPS-374 & 05:41:25.459 & -07:55:18.80 & 0.22 & 56.90 & 0 & 78.2 & 430.5\\
HOPS-261-A & HOPS-261 & 05:41:18.889 & -07:55:28.57 & 2.43 & 149.50 & I & 61.1 & 429.8\\
HOPS-261-B & HOPS-261 & 05:41:18.894 & -07:55:29.34 & 2.43 & 149.50 & I & 61.1 & 429.8\\
HOPS-257 & HOPS-257 & 05:41:19.897 & -07:55:46.77 & 0.34 & 292.60 & Flat & 53.7 & 430.0\\
HOPS-273 & HOPS-273 & 05:40:20.905 & -07:56:24.58 & 2.22 & 243.30 & I & 7.8 & 419.4\\
HOPS-247 & HOPS-247 & 05:41:26.187 & -07:56:51.91 & 3.26 & 42.80 & 0 & 42.4 & 430.9\\
HOPS-248-B & HOPS-248 & 05:41:22.128 & -07:58:02.95 & 2.19 & 484.30 & Flat & 23.7 & 430.7\\
HOPS-248-A & HOPS-248 & 05:41:22.138 & -07:58:03.08 & 2.19 & 484.30 & Flat & 23.7 & 430.7\\
HOPS-245 & HOPS-245 & 05:41:22.892 & -07:58:56.00 & 0.29 & 302.10 & Flat & 18.8 & 431.0\\
HOPS-264 & HOPS-264 & 05:40:59.115 & -08:00:14.40 & 0.06 & 402.30 & Flat & 6.2 & 428.3\\
HOPS-268 & HOPS-268 & 05:40:38.357 & -08:00:36.03 & 1.09 & 113.90 & I & 6.7 & 424.3\\
HOPS-241 & HOPS-241 & 05:41:26.453 & -08:01:02.08 & 0.74 & 100.30 & I & 14.6 & 431.8\\
HOPS-240 & HOPS-240 & 05:41:25.988 & -08:01:15.85 & 0.08 & 191.00 & I & 16.2 & 431.8\\
HOPS-234 & HOPS-234 & 05:41:49.961 & -08:01:26.27 & 2.43 & 79.80 & I & 7.6 & 432.7\\
HOPS-284 & HOPS-284 & 05:38:51.499 & -08:01:27.46 & 0.64 & 913.90 & Flat & 0.7 & 403.4\\
HOPS-238 & HOPS-238 & 05:41:26.657 & -08:03:12.61 & 0.39 & 269.10 & I & 15.6 & 432.2\\
HOPS-237 & HOPS-237 & 05:41:28.984 & -08:03:25.95 & 0.28 & 177.70 & I & 15.8 & 432.5\\
HOPS-236 & HOPS-236 & 05:41:30.223 & -08:03:41.46 & 5.16 & 332.80 & Flat & 14.4 & 432.6\\
HOPS-251 & HOPS-251 & 05:40:54.017 & -08:05:13.18 & 0.66 & 345.70 & Flat & 63.8 & 428.7\\
HOPS-405 & HOPS-405 & 05:40:58.552 & -08:05:34.52 & 1.67 & 35.00 & 0 & 44.0 & 429.3\\
HOPS-255-B & HOPS-255 & 05:40:50.567 & -08:05:48.57 & 0.66 & 572.00 & Flat & 83.2 & 428.4\\
HOPS-255-A & HOPS-255 & 05:40:50.576 & -08:05:48.70 & 0.66 & 572.00 & Flat & 83.2 & 428.4\\
HOPS-249 & HOPS-249 & 05:40:52.869 & -08:05:48.91 & 0.08 & 268.50 & Flat & 72.7 & 428.7\\
HOPS-235 & HOPS-235 & 05:41:25.354 & -08:05:54.70 & 5.06 & 680.10 & Flat & 9.8 & 432.6\\
HOPS-244 & HOPS-244 & 05:41:02.010 & -08:06:01.91 & 1.45 & 127.30 & I & 23.5 & 429.9\\
HOPS-252 & HOPS-252 & 05:40:49.914 & -08:06:08.43 & 1.91 & 329.20 & Flat & 114.7 & 428.5\\
HOPS-256 & HOPS-256 & 05:40:45.274 & -08:06:42.20 & 0.11 & 72.40 & 0 & 83.2 & 427.7\\
HOPS-243 & HOPS-243 & 05:41:01.663 & -08:06:44.60 & 0.45 & 50.80 & 0 & 23.3 & 430.0\\
HOPS-250 & HOPS-250 & 05:40:48.849 & -08:06:57.10 & 7.07 & 69.40 & 0 & 92.0 & 428.5\\
HOPS-250-B & HOPS-250 & 05:40:46.618 & -08:07:12.84 & 7.07 & 69.40 & 0 & 83.2 & 428.5\\
HOPS-232 & HOPS-232 & 05:41:35.471 & -08:08:22.70 & 1.17 & 187.90 & I & 4.0 & 434.0\\
HOPS-246 & HOPS-246 & 05:40:47.112 & -08:09:48.04 & 0.40 & 95.60 & I & 14.1 & 429.1\\
HOPS-242-A & HOPS-242 & 05:40:48.530 & -08:11:08.90 & 0.65 & 836.70 & Flat & 7.9 & 429.6\\
HOPS-242-B & HOPS-242 & 05:40:48.549 & -08:11:08.93 & 0.65 & 836.70 & Flat & 7.9 & 429.6\\
HOPS-259-A & HOPS-259 & 05:40:20.904 & -08:13:55.20 & 0.79 & 410.30 & Flat & 3.8 & 425.3\\
HOPS-259-B & HOPS-259 & 05:40:20.933 & -08:14:06.44 & 0.79 & 410.30 & Flat & 3.8 & 425.3\\
HOPS-260 & HOPS-260 & 05:40:19.400 & -08:14:16.29 & 1.73 & 600.10 & Flat & 3.4 & 425.1\\
HOPS-397 & HOPS-397 & 05:42:49.002 & -08:16:10.68 & 1.75 & 46.10 & 0 & 30.0 & 431.7\\
HOPS-223 & HOPS-223 & 05:42:48.491 & -08:16:34.68 & 20.35 & 247.50 & I & 33.2 & 431.8\\
HOPS-221 & HOPS-221 & 05:42:47.067 & -08:17:06.91 & 8.85 & 172.30 & I & 26.1 & 432.0\\
HOPS-215 & HOPS-215 & 05:43:09.583 & -08:29:27.23 & 0.58 & 195.50 & I & 3.3 & 432.5\\
HOPS-216 & HOPS-216 & 05:42:55.566 & -08:32:48.36 & 0.71 & 117.70 & I & 8.6 & 433.8\\
HOPS-228 & HOPS-228 & 05:41:34.183 & -08:35:27.87 & 12.00 & 293.00 & I & 9.2 & 439.2\\
HOPS-214 & HOPS-214 & 05:42:47.232 & -08:36:36.88 & 0.15 & 360.80 & Flat & 30.4 & 435.0\\
HOPS-211 & HOPS-211 & 05:42:58.340 & -08:37:44.25 & 0.27 & 87.90 & Flat & 45.1 & 434.5\\
HOPS-227 & HOPS-227 & 05:41:32.340 & -08:37:55.54 & 0.37 & 371.00 & Flat & 29.9 & 439.8\\
HOPS-210 & HOPS-210 & 05:42:58.285 & -08:38:05.26 & 1.40 & 204.90 & Flat & 53.7 & 434.6\\
HOPS-213-B & HOPS-213 & 05:42:48.077 & -08:40:08.28 & 1.58 & 534.90 & Flat & 68.4 & 435.6\\
HOPS-213-A & HOPS-213 & 05:42:48.088 & -08:40:08.47 & 1.58 & 534.90 & Flat & 68.4 & 435.6\\
HOPS-224 & HOPS-224 & 05:41:32.066 & -08:40:09.77 & 3.28 & 48.60 & 0 & 29.8 & 440.3\\
HOPS-225 & HOPS-225 & 05:41:30.343 & -08:40:17.73 & 0.92 & 432.50 & Flat & 34.5 & 440.5\\
HOPS-220 & HOPS-220 & 05:41:29.786 & -08:42:46.21 & 0.29 & 193.60 & I & 19.2 & 441.0\\
HOPS-219 & HOPS-219 & 05:41:29.289 & -08:43:04.31 & 2.25 & 90.00 & I & 18.1 & 441.1\\
HOPS-208 & HOPS-208 & 05:42:52.733 & -08:44:13.11 & 0.02 & 373.50 & Flat & 10.9 & 436.1\\
HOPS-206 & HOPS-206 & 05:43:07.293 & -08:44:31.27 & 2.47 & 65.10 & 0 & 5.7 & 435.2\\
HOPS-204 & HOPS-204 & 05:43:10.185 & -08:46:07.86 & 1.44 & 85.40 & I & 4.1 & 435.4\\


==> multiples-input-catalog-perseus.tex <==
Per-emb-53 & Per-emb-53 & 03:47:41.591 & +32:51:43.67 & 8.00 & 287.00 & I & 0.6\\
Per-emb-56 & Per-emb-56 & 03:47:05.450 & +32:43:08.24 & 0.92 & 312.00 & I & 1.4\\
IRAS 03363+3207 & IRAS 03363+3207 & 03:39:25.546 & +32:17:07.08 & -99.00 & -99.00 & Unclassified & 0.6\\
EDJ2009-385 & EDJ2009-385 & 03:44:18.168 & +32:04:56.90 & 0.65 & 1200.00 & II & 93.7\\
Per-emb-16 & Per-emb-16 & 03:43:50.978 & +32:03:24.10 & 0.68 & 39.00 & 0 & 162.5\\
Per-emb-11-C & Per-emb-11 & 03:43:57.687 & +32:03:09.97 & 2.55 & 30.00 & 0 & 360.9\\
Per-emb-28 & Per-emb-28 & 03:43:51.007 & +32:03:08.04 & 1.19 & 45.00 & 0 & 201.0\\
Per-emb-11-A & Per-emb-11 & 03:43:57.064 & +32:03:04.78 & 2.55 & 30.00 & 0 & 360.9\\
Per-emb-11-B & Per-emb-11 & 03:43:56.881 & +32:03:02.97 & 2.55 & 30.00 & 0 & 360.9\\
Per-emb-32-A & Per-emb-32 & 03:44:02.403 & +32:02:04.75 & 0.51 & 57.00 & 0 & 285.1\\
Per-emb-32-B & Per-emb-32 & 03:44:02.632 & +32:01:59.43 & 0.51 & 57.00 & 0 & 285.1\\
EDJ2009-366 & EDJ2009-366 & 03:43:59.650 & +32:01:54.00 & 3.06 & 620.00 & II & 227.1\\
Per-emb-62 & Per-emb-62 & 03:44:12.976 & +32:01:35.41 & 3.06 & 378.00 & I & 168.8\\
Per-emb-8 & Per-emb-8 & 03:44:43.981 & +32:01:35.21 & 4.42 & 43.00 & 0 & 93.6\\
Per-emb-55-B & Per-emb-55 & 03:44:43.333 & +32:01:31.63 & 3.06 & 309.00 & I & 101.0\\
Per-emb-55-A & Per-emb-55 & 03:44:43.297 & +32:01:31.22 & 3.06 & 309.00 & I & 101.0\\
Per-emb-1 & Per-emb-1 & 03:43:56.805 & +32:00:50.20 & 3.06 & 27.00 & 0 & 170.5\\
Per-emb-61 & Per-emb-61 & 03:44:21.357 & +31:59:32.51 & 0.41 & 371.00 & I & 146.6\\
Per-emb-9 & Per-emb-9 & 03:29:51.832 & +31:39:05.90 & 1.02 & 36.00 & 0 & 4.5\\
Per-emb-19 & Per-emb-19 & 03:29:23.497 & +31:33:29.17 & 0.61 & 60.00 & 0 & 18.1\\
Per-emb-23 & Per-emb-23 & 03:29:17.211 & +31:27:46.30 & 1.36 & 42.00 & 0 & 88.4\\
EDJ2009-235 & EDJ2009-235 & 03:29:18.258 & +31:23:19.75 & 0.92 & -99.00 & II & 366.3\\
Per-emb-57 & Per-emb-57 & 03:29:03.331 & +31:23:14.57 & 0.15 & 313.00 & I & 359.7\\
Per-emb-37 & Per-emb-37 & 03:29:18.964 & +31:23:14.30 & 0.85 & 22.00 & 0 & 312.1\\
EDJ2009-233 & EDJ2009-233 & 03:29:17.675 & +31:22:44.92 & 2.38 & 1300.00 & II & 395.3\\
Per-emb-65 & Per-emb-65 & 03:28:56.316 & +31:22:27.79 & 0.27 & 440.00 & I & 354.5\\
Per-emb-58 & Per-emb-58 & 03:28:58.422 & +31:22:17.48 & 1.07 & 322.00 & I & 540.6\\
SVS3 & SVS3 & 03:29:10.419 & +31:21:59.07 & 0.92 & -99.00 & II & 643.5\\
Per-emb-50 & Per-emb-50 & 03:29:07.768 & +31:21:57.12 & 39.47 & 128.00 & I & 610.2\\
Per-emb-64 & Per-emb-64 & 03:33:12.851 & +31:21:24.02 & 5.44 & 438.00 & I & 5.3\\
Per-emb-54 & Per-emb-54 & 03:29:01.549 & +31:20:20.49 & 28.58 & 131.00 & I & 379.2\\
EDJ2009-172 & EDJ2009-172 & 03:28:56.649 & +31:18:35.44 & 0.66 & 1100.00 & II & 272.7\\
Per-emb-18-B & Per-emb-18 & 03:29:11.261 & +31:18:31.07 & 4.76 & 59.00 & 0 & 202.9\\
Per-emb-18-A & Per-emb-18 & 03:29:11.254 & +31:18:31.05 & 4.76 & 59.00 & 0 & 202.9\\
Per-emb-21 & Per-emb-21 & 03:29:10.668 & +31:18:20.19 & 11.74 & 45.00 & 0 & 193.9\\
EDJ2009-156-A & EDJ2009-156-A & 03:28:51.031 & +31:18:18.38 & 0.07 & 740.00 & II & 315.2\\
EDJ2009-156-B & EDJ2009-156-B & 03:28:51.111 & +31:18:15.44 & 0.07 & 740.00 & II & 308.2\\
Per-emb-49-B & Per-emb-49 & 03:29:12.975 & +31:18:14.39 & 1.87 & 239.00 & I & 175.3\\
Per-emb-49-A & Per-emb-49 & 03:29:12.952 & +31:18:14.28 & 1.87 & 239.00 & I & 175.3\\
Per-emb-63 & Per-emb-63 & 03:28:43.270 & +31:17:32.93 & 3.23 & 436.00 & I & 240.7\\
Per-emb-52 & Per-emb-52 & 03:28:39.699 & +31:17:31.88 & 0.27 & 278.00 & I & 132.0\\
EDJ2009-173 & EDJ2009-173 & 03:28:56.963 & +31:16:22.19 & 0.17 & 1100.00 & II & 620.1\\
Per-emb-44-A & Per-emb-44 & 03:29:03.766 & +31:16:03.81 & 55.29 & 188.00 & 0 & 387.0\\
Per-emb-44-B & Per-emb-44 & 03:29:03.742 & +31:16:03.78 & 55.29 & 188.00 & 0 & 387.0\\
SVS13A2 & SVS13A2 & 03:29:03.386 & +31:16:01.62 & 0.17 & 20.00 & 0 & 431.0\\
SVS13B & SVS13B & 03:29:03.077 & +31:15:51.73 & 1.70 & 20.00 & 0 & 505.8\\
EDJ2009-183-A & EDJ2009-183-A & 03:28:59.295 & +31:15:48.40 & 5.44 & 100.00 & I & 668.5\\
EDJ2009-183-B & EDJ2009-183-B & 03:28:59.373 & +31:15:48.39 & 5.44 & 100.00 & I & 668.5\\
SVS13C & SVS13C & 03:29:01.970 & +31:15:38.05 & 2.55 & 21.00 & 0 & 496.1\\
Per-emb-15 & Per-emb-15 & 03:29:04.054 & +31:14:46.23 & 0.68 & 36.00 & 0 & 299.6\\
Per-emb-27-A & Per-emb-27 & 03:28:55.569 & +31:14:37.02 & 32.33 & 69.00 & 0 & 254.6\\
Per-emb-27-B & Per-emb-27 & 03:28:55.563 & +31:14:36.40 & 32.33 & 69.00 & 0 & 254.6\\
BD-+30-547 & BD-+30-547 & 03:28:57.222 & +31:14:18.99 & 0.94 & 5000.00 & Unclassified & 208.9\\
Per-emb-36-B & Per-emb-36 & 03:28:57.370 & +31:14:16.07 & 9.02 & 106.00 & I & 209.1\\
Per-emb-36-A & Per-emb-36 & 03:28:57.373 & +31:14:15.76 & 9.02 & 106.00 & I & 209.1\\
Per-emb-14 & Per-emb-14 & 03:29:13.547 & +31:13:58.15 & 1.19 & 31.00 & 0 & 179.8\\
Per-emb-12-B & Per-emb-12 & 03:29:10.427 & +31:13:32.09 & 11.91 & 29.00 & 0 & 160.7\\
Per-emb-35-B & Per-emb-35 & 03:28:37.219 & +31:13:31.75 & 15.48 & 103.00 & I & 50.3\\
Per-emb-12-A & Per-emb-12 & 03:29:10.536 & +31:13:30.92 & 11.91 & 29.00 & 0 & 160.7\\
Per-emb-35-A & Per-emb-35 & 03:28:37.090 & +31:13:30.78 & 15.48 & 103.00 & I & 50.3\\
Per-emb-13 & Per-emb-13 & 03:29:12.015 & +31:13:08.03 & 6.81 & 28.00 & 0 & 157.2\\
IRAS 4B' & IRAS 4B' & 03:29:12.841 & +31:13:06.89 & 0.17 & 15.00 & 0 & 158.7\\
Per-emb-3 & Per-emb-3 & 03:29:00.574 & +31:12:00.20 & 0.85 & 32.00 & 0 & 120.3\\
Per-emb-31 & Per-emb-31 & 03:28:32.547 & +31:11:05.15 & 0.27 & 80.00 & 0 & 23.2\\
Per-emb-29 & Per-emb-29 & 03:33:17.877 & +31:09:31.81 & 6.29 & 48.00 & 0 & 44.0\\
Per-emb-40-B & Per-emb-40 & 03:33:16.679 & +31:07:55.26 & 2.55 & 132.00 & I & 49.4\\
Per-emb-40-A & Per-emb-40 & 03:33:16.669 & +31:07:54.90 & 2.55 & 132.00 & I & 49.4\\
B1-bN & B1-bN & 03:33:21.209 & +31:07:43.66 & 0.54 & 14.70 & 0 & 62.5\\
B1-bS & B1-bS & 03:33:21.355 & +31:07:26.37 & 1.19 & 17.70 & 0 & 55.3\\
Per-emb-41 & Per-emb-41 & 03:33:20.341 & +31:07:21.35 & 0.29 & 157.00 & I & 50.5\\
Per-emb-6 & Per-emb-6 & 03:33:14.404 & +31:07:10.71 & 0.51 & 52.00 & 0 & 62.6\\
Per-emb-30 & Per-emb-30 & 03:33:27.303 & +31:07:10.15 & 2.89 & 78.00 & 0 & 41.1\\
Per-emb-10 & Per-emb-10 & 03:33:16.424 & +31:06:52.06 & 1.02 & 30.00 & 0 & 52.3\\
Per-emb-24 & Per-emb-24 & 03:28:45.297 & +31:05:41.69 & 0.73 & 67.00 & 0 & 18.4\\
Per-emb-38 & Per-emb-38 & 03:32:29.197 & +31:02:40.75 & 0.92 & 115.00 & I & 11.1\\
IRAS 03295+3050 & IRAS 03295+3050 & 03:32:34.066 & +31:00:55.62 & 0.43 & 1300.00 & II & 8.6\\
Per-emb-47 & Per-emb-47 & 03:28:34.507 & +31:00:50.99 & 2.04 & 230.00 & I & 8.1\\
Per-emb-2-B & Per-emb-2 & 03:32:17.926 & +30:49:47.75 & 1.53 & 27.00 & 0 & 4.2\\
Per-emb-2-A & Per-emb-2 & 03:32:17.931 & +30:49:47.70 & 1.53 & 27.00 & 0 & 4.2\\
L1448IRS1-A & L1448IRS1-A & 03:25:09.449 & +30:46:21.92 & -99.00 & -99.00 & I & 24.8\\
L1448IRS1-B & L1448IRS1-B & 03:25:09.412 & +30:46:20.62 & -99.00 & -99.00 & I & 24.8\\
L1448NW-B & L1448NW-B & 03:25:35.672 & +30:45:34.35 & 2.38 & 22.00 & 0 & 171.3\\
L1448NW-A & L1448NW-A & 03:25:35.669 & +30:45:34.10 & 2.38 & 22.00 & 0 & 171.6\\
Per-emb-5-A & Per-emb-5 & 03:31:20.942 & +30:45:30.26 & 2.21 & 32.00 & 0 & 3.8\\
Per-emb-5-B & Per-emb-5 & 03:31:20.934 & +30:45:30.24 & 2.21 & 32.00 & 0 & 3.8\\
L1448IRS3A & L1448IRS3A & 03:25:36.499 & +30:45:21.88 & 15.65 & 47.00 & I & 153.3\\
Per-emb-33-B & Per-emb-33 & 03:25:36.312 & +30:45:15.15 & 14.12 & 57.00 & 0 & 159.6\\
Per-emb-33-C & Per-emb-33 & 03:25:36.321 & +30:45:14.91 & 14.12 & 57.00 & 0 & 159.6\\
Per-emb-33-A & Per-emb-33 & 03:25:36.380 & +30:45:14.72 & 14.12 & 57.00 & 0 & 159.6\\
Per-emb-22-A & Per-emb-22 & 03:25:22.409 & +30:45:13.25 & 6.12 & 43.00 & 0 & 72.9\\
Per-emb-22-B & Per-emb-22 & 03:25:22.352 & +30:45:13.15 & 6.12 & 43.00 & 0 & 72.9\\
Per-emb-26 & Per-emb-26 & 03:25:38.874 & +30:44:05.28 & 14.29 & 47.00 & 0 & 69.1\\
Per-emb-42 & Per-emb-42 & 03:25:39.135 & +30:43:57.90 & 1.16 & 163.00 & I & 63.8\\
EDJ2009-269-A & EDJ2009-269-A & 03:30:44.013 & +30:32:46.81 & 2.21 & 1200.00 & II & 3.8\\
EDJ2009-269-B & EDJ2009-269-B & 03:30:43.978 & +30:32:46.57 & 2.21 & 1200.00 & II & 3.8\\
EDJ2009-263 & EDJ2009-263 & 03:30:27.161 & +30:28:29.61 & 0.39 & 340.00 & I & 2.8\\
L1451-MMS & L1451-MMS & 03:25:10.244 & +30:23:55.05 & 0.09 & 15.00 & 0 & 1.7\\
Per-emb-34 & Per-emb-34 & 03:30:15.162 & +30:23:49.23 & 2.72 & 99.00 & I & 2.9\\
Per-emb-25 & Per-emb-25 & 03:26:37.510 & +30:15:27.81 & 2.04 & 61.00 & 0 & 4.0\\
Per-emb-48-A & Per-emb-48 & 03:27:38.277 & +30:13:58.55 & 1.48 & 238.00 & I & 14.7\\
Per-emb-48-B & Per-emb-48 & 03:27:38.258 & +30:13:58.31 & 1.48 & 238.00 & I & 14.7\\
Per-emb-17-A & Per-emb-17 & 03:27:39.104 & +30:13:03.07 & 7.15 & 59.00 & 0 & 16.1\\
Per-emb-17-B & Per-emb-17 & 03:27:39.115 & +30:13:02.83 & 7.15 & 59.00 & 0 & 16.1\\
Per-emb-20 & Per-emb-20 & 03:27:43.276 & +30:12:28.78 & 2.38 & 65.00 & 0 & 13.9\\
L1455IRS2 & L1455IRS2 & 03:27:47.689 & +30:12:04.31 & 4.25 & 740.00 & I & 12.2\\
Per-emb-46 & Per-emb-46 & 03:28:00.414 & +30:08:01.01 & 0.51 & 221.00 & I & 5.1\\

